All-atomic source of squeezed vacuum with full pulse-shape control

We report on the generation of pulses of a low-frequency squeezed vacuum with noise suppression >2 dB below the standard quantum limit in a hot resonant 87 Rb vapor with polarization self-rotation. We demonstrate the possibility to precisely control the temporal profile of the squeezed noise quadrature by applying a calibrated longitudinal magnetic field, without degrading the maximum amount of squeezing.

==> Makefile <==
# -*- make -*-
# FILE: "/home/evmik/jobs/paper/drafts/squeezing_pulses/Makefile"
# LAST MODIFICATION: "Fri, 20 Jan 2012 14:07:00 -0500 (evmik)"
# (C) 2001 by Eugeniy Mikhailov, <evmik@tamu.edu>
# $Id: Makefile,v 1.3 2003/04/23 20:40:19 evmik Exp $

SUBDIR=`find ./ -maxdepth 1 -type d |sed 1d| sed /CVS/d`

LATEX_OPTIONS="-interaction=nonstopmode -src-specials"
COLOR_TYPE_FILE=mode_type.in


EPS_PICTURES=

DATE := $(shell date +%Y%m%d)

ROOT_OF_MAIN_TEX_FILE= sqzpulse
MAIN_TEX_FILE=$(ROOT_OF_MAIN_TEX_FILE).tex

source_files  = $(wildcard *.tex)
source_basename = $(source_files:%.tex=%)

tex_targets  = $(wildcard *.tex)
pdf_targets  = $(tex_targets:%.tex=%.pdf)	
ps_targets  = $(tex_targets:%.tex=%.ps)	
dvi_targets  = $(tex_targets:%.tex=%.dvi)	

default: dvi

INCLUDED_TEX_FILES=bibliography.bib


$(INCLUDED_TEX_FILES):
	 

$(EPS_PICTURES): 
	action=ps; \
	for d in $(SUBDIR); \
	do \
		root_dir=`pwd` ; \
		cd $$d;  make $${action}; \
		cd $$root_dir ; \
	done
	
force_eps:
	action=ps; \
	for d in $(SUBDIR); \
	do \
		root_dir=`pwd` ; \
		cd $$d;  make $${action}; \
		cd $$root_dir ; \
	done

pdf_pictures:
	action=pdf; \
	for d in $(SUBDIR); \
	do \
		root_dir=`pwd` ; \
		cd $$d;  make $${action}; \
		cd $$root_dir ; \
	done


eps:  $(EPS_PICTURES)

dvi: $(dvi_targets)

$(dvi_targets):  %.dvi : %.tex
	rubber $<


ps:	$(ps_targets)

$(ps_targets).ps: %.ps : %.dvi
	dvips -o $@ $<


2page: ps
	psnup -n 2 -pletter $(ROOT_OF_MAIN_TEX_FILE).ps > $(ROOT_OF_MAIN_TEX_FILE)_2pages.ps

pdf: $(pdf_targets)

#home of  dvipdfm utilit is at
#http://gaspra.kettering.edu/dvipdfm/
# optimized for 'dvipdfm'
$(pdf_targets): %.pdf : %.dvi 
	dvipdfmx $<




zip:
	zip -r arch.$(ROOT_OF_MAIN_TEX_FILE).`date +%F`.zip  $(ROOT_OF_MAIN_TEX_FILE).tex Makefile bibliography.bib figures ol.bst osajnl.bst osajnl2.rtx osajnl2.sty `tex2figlist.sh $(ROOT_OF_MAIN_TEX_FILE).tex`

clean_results:
	rm -f $(pdf_targets)
	
clean: clean_tex clean_bib clean_backups
	rm -f $(ROOT_OF_MAIN_TEX_FILE).tar.gz
	action="clean" ; \
	for d in $(SUBDIR); \
	do \
		root_dir=`pwd` ; \
		cd $$d;  make $${action}; \
		cd $$root_dir ; \
	done

real_clean: clean_all

clean_backups:
	rm -f *~

clean_tex:
	rm -f $(tex_targets:%.tex=%.dvi)
	rm -f $(tex_targets:%.tex=%.log)
	rm -f $(tex_targets:%.tex=%.aux)
	rm -f $(tex_targets:%.tex=%.nav)
	rm -f $(tex_targets:%.tex=%.out)
	rm -f $(tex_targets:%.tex=%.snm)
	rm -f $(tex_targets:%.tex=%.toc)
	rm -f $(tex_targets:%.tex=%.vrb)
	rm -f $(tex_targets:%.tex=%.blg)
	rm -f missfont.log

clean_bib:
	rm -f $(tex_targets:%.tex=%.bbl)

clean_for_arxive: clean_results clean_backups clean_tex

clean_all: clean clean_results clean_backups

arxive_submission: $(ROOT_OF_MAIN_TEX_FILE).for_arxive.$(DATE).tar.gz

$(ROOT_OF_MAIN_TEX_FILE).for_arxive.$(DATE).tar.gz: clean_for_arxive
	cd ..; tar c --dereference --exclude=.git --exclude=*gz squeezing_pulses |gzip > $@
	mv ../$@ .


arch:
	cd ..; tar c --dereference --exclude=.git --exclude=*gz squeezing_pulses |gzip > $(ROOT_OF_MAIN_TEX_FILE).$(DATE).tar.gz
	mv ../$(ROOT_OF_MAIN_TEX_FILE).$(DATE).tar.gz .


figures.lst:
	multidir_tex2onedir.sh $(ROOT_OF_MAIN_TEX_FILE).tex  tmp_dir do_not_change_pics_name
	rm -r tmp_dir

upload_draft_to_web:
	rsync --delete -avze ssh ../squeezing_pulses physics.wm.edu:public_html/drafts/


